Amadeus: Scalable, Privacy-Preserving Live Video Analytics

Smart-city applications ranging from traffic management to public-safety alerts rely on live analytics of video from surveillance cameras in public spaces. However, a growing number of government regulations stipulate how data collected from these cameras must be handled in order to protect citizens' privacy. This paper describes Amadeus, which balances privacy and utility by redacting video in near realtime for smart-city applications. Our main insight is that whitelisting objects, or blocking by default, is crucial for scalable, privacy-preserving video analytics. In the context of modern object detectors, we prove that whitelisting reduces the risk of an object-detection error leading to a privacy violation, and helps Amadeus scale to a large and diverse set of applications. In particular, Amadeus utilizes whitelisting to generate composable encrypted object-specific live streams, which simultaneously meet the requirements of multiple applications in a privacy-preserving fashion, while reducing the compute and streaming-bandwidth requirements at the edge. Experiments with our Amadeus prototype show that compared to blacklisting objects, whitelisting yields significantly better privacy (up to ~28x) and bandwidth savings (up to ~5.5x). Additionally, our experiments also indicate that the composable live streams generated by Amadeus are usable by real-world applications with minimum utility loss.

==> intro.tex <==
Cameras are ubiquitous. Multiple application domains including but not limited to smart cities \cite{smart-cities}, traffic management \cite{quartz}, pedestrian detection \cite{pedestrian-detection}, public safety \cite{public-safety} and surveillance rely on extracting insights from video streams to \textit{perceive} their environment. These applications can be enabled by utilizing video-analytics frameworks \cite {rocket, focus, noscope} which extract useful information by utilizing object detection \cite{yolo, faster-rcnn} and tracking \cite{sort, opencv-tracker} techniques. These frameworks generally annotate frames with metadata of the detected objects, which can be used to (i) provide per-frame insights \cite{noscope}, (ii) answer \textit{after-the-fact} queries \cite{focus}, and/or (iii) provide a notification in response to detecting an event of a pre-specified type. 

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{images/defocus-motivation.pdf} % Example image
	\vspace{-0.3cm}
	\textbf{\caption{\system: Privacy-Preserving Live Streaming}}
	\label{fig:defocus-motivation}
\end{figure}

Privacy is an important concern as most cameras are deployed in public spaces. If an unauthorized user is able to glean personally-identifiable information from a video stream, there is a possibility of personal harm or financial loss. Consider publicly-available online video streams \cite{seattle, jackson-hole}. The primary objective of making these streams available is to give commuters an idea of the traffic congestion at a given location. However, these streams can also be misused by malicious actors to detect and track both persons and objects. This opens up the possibility of a person's residential/work address or their location at a specific time of day being revealed. 

While unauthorized video-analytics is a concern, it can be prevented by utilizing authentication and access-control mechanisms \cite{authentication}. Instead, an increasing cause of worry is authorized users going beyond their mandate or publicly-specified objective. Consider a common smart-city scenario, where a video stream originating at a camera may be \textit{consumed} by separate entities, each with their own mandate. For example, consumer \textsf{A} is mandated to analyze vehicles to measure traffic congestion, consumer \textsf{B} is mandated to count pedestrians to decide an appropriate pedestrian-crossing duration, and consumer \textsf{C} is mandated to count the number of bicycles. Note that these consumers could be automated applications or human viewers. In this scenario, consumers \textsf{A} and \textsf{C} are not mandated to perform any analysis on persons observed in the video. However, malicious actors can go beyond their mandate and perform facial recognition on the video stream. In such a case, there is no way for the owner or administrator of the video stream to know if any consumer has \textit{exceeded} their mandate.

To prevent such situations, government entities have instituted policies to preserve privacy \cite{gdpr, san-francisco}. For example, the city of San Francisco introduced a law banning the use of facial recognition on public cameras \cite{san-francisco}. While such policies are desirable to protect the privacy of individuals, there is a need for a mechanism to physically-limit privacy loss, by ensuring that video consumers cannot exceed their specified mandate.

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{images/blacklist-whitelist.pdf} % Example image
	\vspace{-0.3cm}
	\caption{Blacklisting v/s Whitelisting in the context of a vehicle-counting application}
	\label{fig:blacklist-whitelist}
\end{figure}

While privacy is of paramount importance, we also need to satisfy the requirements of each consumer, such that they can meet their mandate. This leads to a situation, where we need to perform privacy-preserving transformations on the raw video stream to create a custom video stream for each consumer at ingest time. Two important types of privacy-preserving transformations are as follows:
\begin{itemize}[noitemsep]
	\item \textbf{Blacklisting:} also known as the \textit{allow-by-default} approach, redacts all objects belonging to sensitive classes from the video stream. 
	\item \textbf{Whitelisting:} also known as the \textit{block-by-default} approach, selectively discloses \textit{only} the objects of relevant classes in the video stream, that a consumer requires to perform her specified mandate. 
\end{itemize}

Figure \ref{fig:blacklist-whitelist} contrasts blacklisting and whitelisting using an example vehicle-counting application. To count vehicles in a scene, while preserving privacy, an application requires to view only objects corresponding to vehicles in the scene. Therefore, the whitelisting approach will only disclose objects belonging to classes \quotes{car} and \quotes{truck}, while all other content is \textit{blocked} by default. On the other hand, to preserve privacy, the blacklisting approach will disclose all information in the video stream to the application \textit{except} those belonging to the sensitive class \quotes{person}, which will be redacted.

Both of the above-mentioned privacy-preserving transformations rely on object detection. Therefore, the same object-detection mechanism used to extract analytics from videos at ingest time, can also be used to \textit{generate} privacy-preserving streams. The emergence of edge computing \cite{edge-computing-satya} has made it possible to perform these object-detection-based transformations at the camera or one-network-hop-away from the camera. However, while an edge-computing-platform may have sufficient resources to process video frames in real time, network bandwidth at the edge is a scarce and expensive resource \cite{edge-network}. Therefore, it is essential that we support multiple applications, while staying within the compute and network-bandwidth constraints at the edge.

\textbf{Objectives:} We introduce \systembold, a privacy-preserving live-streaming and video-analytics pipeline. The key objectives of \system are as follows: (i) minimize privacy leakage by creating privacy-preserving live video streams such that applications can meet their stated objectives, but not glean any private information, (ii) minimize the bandwidth requirement at the edge, while simultaneously supporting multiple consumer applications with different mandates, and (iii) providing per-frame analytics to consumer applications. 

\textbf{Threat Model:} We assume that our \system pipeline is trusted, is deployed on the camera or on an edge device, and has access to the raw-video feed. All other applications are untrusted, do not have access to the raw stream, and need to consume processed video streams generated by \system.

\textbf{Contributions:} Our contributions are as follows:
%\setlist{nolistsep}
\begin{itemize}[noitemsep]
	\item We show that when using modern object-detection techniques at ingest time, the \textit{block-by-default} or whitelisting approach can yield lower privacy loss as compared to the \textit{allow-by-default} or blacklisting approach.
	\item We introduce a new bandwidth-saving and privacy-preserving streaming mechanism which encodes a single video stream into multiple encrypted \textit{per-object-class} video streams. These component streams can be composed to reconstruct the entire video stream.
	\item We introduce \system, a privacy-preserving live-streaming and video-analytics pipeline. \system favors a \textit{whitelisting} approach to simultaneously support multiple consumer applications, while preserving privacy and minimizing the bandwidth requirement to stream videos from the edge using the \textit{composition} mechanism.
	\item We evaluate the end-to-end resource requirements, privacy-preserving properties, bandwidth requirements and scalability of \system using real-world video data and applications.
\end{itemize}

While the key ideas proposed in this paper are relevant for video streaming, we believe that they are also applicable for other types of content streaming, including audio and text.

This rest of this paper is organized as follows: Section \ref{sec:background} provides some background on object-detection techniques, and highlights its implications on privacy with respect to the whitelisting and blacklisting approaches. Section \ref{sec:design} presents the key ideas which \system utilizes to generate bandwidth-efficient privacy-preserving streams, and Section \ref{sec:implementation} provides implementation details. Finally, Section \ref{sec:evaluation} provides end-to-end evaluation results for \system, Section \ref{sec:related-work} provides a glimpse of relevant prior work, and Section \ref{sec:conclusion} concludes the paper.

